Surface Vision Transformers: Flexible Attention-Based Modelling of Biomedical Surfaces

Recent state-of-the-art performances of Vision Transformers (ViT) in computer vision tasks demonstrate that a general-purpose architecture, which implements long-range self-attention, could replace the local feature learning operations of convolutional neural networks. In this paper, we extend ViTs to surfaces by reformulating the task of surface learning as a sequence-to-sequence learning problem, by proposing patching mechanisms for general surface meshes. Sequences of patches are then processed by a transformer encoder and used for classification or regression. We validate our method on a range of different biomedical surface domains and tasks: brain age prediction in the developing Human Connectome Project (dHCP), fluid intelligence prediction in the Human Connectome Project (HCP), and coronary artery calcium score classification using surfaces from the Scottish Computed Tomography of the Heart (SCOT-HEART) dataset, and investigate the impact of pretraining and data augmentation on model performance. Results suggest that Surface Vision Transformers (SiT) demonstrate consistent improvement over geometric deep learning methods for brain age and fluid intelligence prediction and achieve comparable performance on calcium score classification to standard metrics used in clinical practice. Furthermore, analysis of transformer attention maps offers clear and individualised predictions of the features driving each task. Code is available on Github: https://github.com/metrics-lab/surface-vision-transformers

==> other.tex <==

%% IDEAS
% challenges in studying surfaces; especially in cortical analysis and cardiac; 
% geometric deep learning
% vision transformers
%

%Studying surfaces is challenging in medical imaging, as most of the tools that have been developed are suitable for Euclidean domains but fail to extend to non-Euclidean manifolds. Geometric Deep Learning methods, such as graphs networks, surface and spectral convolutions or point clouds architecture, have been developed for studying such manifolds; however, many fail to adapt to different tasks and datasets. 


% Preserving topological information is critical for many medical imaging tasks \cite{saha2015digital}. Two domains where this is particularly important are magnetic resonance imaging (MRI) of the brain and heart. 



%\subsubsection{dHCP Results}
%\begin{table}[h]
%\centering
%\setlength{\tabcolsep}{6pt}
%\begin{tabular}{lcccc}
%        \toprule
%         \textbf{Methods} & \textbf{Balance} & \textbf{Rotation} & %\textbf{Shuffle} &  \textbf{MAE} \\
%        \midrule
%        SiT-tiny & \cmark & \cmark & n/a & 0.73 $\pm$ \\
%        ChebNet & \cmark & \cmark & n/a & 0.77 $\pm$\\
%        GConvNet & \cmark & \cmark & n/a & 0.75 $\pm$\\
%        Spherical UNet & \cmark & \cmark & n/a & 0.87 $\pm$\\
%        MoNet & \cmark & \cmark & n/a & 0.61 $\pm$\\
%        \midrule
%        \midrule
%        SiT-tiny & \xmark & \xmark & \xmark & 0.77 $\pm$ \\
%        SiT-tiny & \cmark & \xmark & \xmark & xx $\pm$ \\
%        SiT-tiny & \cmark & \cmark & \xmark & xx $\pm$ \\
%        \midrule
%        SiT-small & \xmark & \xmark & \xmark & 0.76 $\pm$\\
%        SiT-small & \cmark & \xmark & \xmark & xx $\pm$ \\
%        SiT-small & \cmark & \cmark & \xmark & xx $\pm$\\
%        \midrule
%        SiT-base & \xmark & \xmark & \xmark & 0.68 $\pm$\\
%        SiT-base & \cmark & \xmark & \xmark & xx $\pm$ \\
%        SiT-base & \cmark & \cmark & \xmark & xx $\pm$\\
%        \bottomrule
%        \\
%\end{tabular}
%\caption{SiT augmentations - PMA predictions - Native dHCP}
%\centering
%\label{Table:sit_augm}
%\end{table}


%\begin{table}[h]
%\centering
%\setlength{\tabcolsep}{6pt}
%\begin{tabular}{lcccc}
%        \toprule
%         \textbf{Methods} & \textbf{Balance} & \textbf{Rotation} & \textbf{Shuffle} &  \textbf{MAE} \\
%        \midrule
%        SiT-tiny & \cmark & \cmark & n/a & 1.52 $\pm$ \\
%        ChebNet & \cmark & \cmark & n/a & 1.70 $\pm$\\
%        GConvNet & \cmark & \cmark & n/a & 2.30 $\pm$\\
%        Spherical UNet & \cmark & \cmark & n/a & 2.16 $\pm$\\
%        MoNet & \cmark & \cmark & n/a & 1.58 $\pm$\\
%        \midrule
%        \midrule
%        SiT-tiny & \xmark & \xmark & \xmark & 1.75 $\pm$ \\
%        SiT-tiny & \cmark & \xmark & \xmark & 1.39 $\pm$ \\
%        SiT-tiny & \cmark & \cmark & \xmark & 1.36 $\pm$ \\
%       \midrule
%        SiT-small & \xmark & \xmark & \xmark & 1.72 $\pm$\\
%        SiT-small & \cmark & \xmark & \xmark & 1.47 $\pm$ \\
%        SiT-small & \cmark & \cmark & \xmark & 1.22 $\pm$\\\midrule
%        SiT-base & \xmark & \xmark & \xmark & 1.63 $\pm$\\
%        SiT-base & \cmark & \xmark & \xmark & 1.59 $\pm$ \\
%        SiT-base & \cmark & \cmark & \xmark & 1.21 $\pm$\\
%        \bottomrule
%        \\
%\end{tabular}
%\caption{SiT augmentations - GA predictions - Native dHCP}
%\centering
%\label{Table:sit_augm}
%\end{table}

%\begin{table*}[h]
%  \footnotesize
%  \centering
%  \setlength{\tabcolsep}{10pt}
%  \renewcommand{\arraystretch}{1.15}
%  \begin{tabular}{l|c|c|c|c|c|c|c}
%    \hline
%    \multirow{2}{1.2cm}{\textbf{Methods}} &\multirow{2}{1.5cm}{\textbf{Pretraining}} &\multirow{2}{1.7cm}{\textbf{Augmentation}}  %&\multicolumn{2}{c|}{\textbf{PMA}} & \multicolumn{2}{c|}{\textbf{GA - deconfounded}}  &\multirow{2}{1.0cm}{\textbf{Average}}\\
%    \cline{4-7}
%    &&&  \textbf{Template} & \textbf{Native}&   \textbf{Template} &\textbf{Native} \\
%    \hline
%    \hline
%    S2CNN &\xmark & \xmark  & 0.63 $\pm0.02$& 0.73 $\pm0.25$  & 1.35 $\pm0.68$& 1.52 $\pm0.60$&1.06\\
%    ChebNet &\xmark & \xmark  & 0.59 $\pm0.37$ & 0.77 $\pm0.49$& 1.57 $\pm0.15$& 1.70 $\pm0.36$& 1.16\\
%    GConvNet &\xmark & \xmark   & 0.75 $\pm0.13$& 0.75 $\pm0.26$& 1.77 $\pm0.26$& 2.30 $\pm0.74$&1.39\\
%    Spherical UNet & \xmark & \xmark  & 0.57 $\pm0.18$& 0.87 $\pm0.50$& \textbf{0.85} $\pm0.17$& 2.16 $\pm0.57$&1.11\\
%    MoNet & \xmark & \xmark  & 0.57 $\pm0.02$ & \textbf{0.61} $\pm0.05$&   1.44 $\pm0.08$&1.58 $\pm0.06$&1.05\\
%    \hline
%    SiT-tiny & \xmark & \xmark& 0.63 $\pm$0.01  & 0.77 $\pm$0.03 & 1.43 $\pm$0.01 & 1.75 $\pm$0.14& 1.15\\
%    SiT-tiny &  \cmark& \xmark& 0.58 $\pm$0.01 & 0.64 $\pm$0.06  & 1.40 $\pm$0.23 & 1.70 $\pm$0.10&1.08\\
%    SiT-small &  \xmark& \xmark & 0.60 $\pm$0.02& 0.76 $\pm$0.03  & 1.14 $\pm$0.12 & 1.44 $\pm$0.03&0.99\\
%    SiT-small &  \cmark& \xmark& \textbf{0.55} $\pm$0.04& 0.63 $\pm$0.06 & 1.25 $\pm$0.06& \textbf{1.21} $\pm$0.22&0.91\\
%    \hline
%    \hline
%    S2CNN &\xmark & \cmark  & 0.63 $\pm0.02$& 0.79 $\pm0.20$  & 1.55 $\pm0.46$& 1.67 $\pm0.40$&1.16\\
%    ChebNet &\xmark & \cmark  & 0.64 $\pm0.01$ & 0.68 $\pm0.41$& 1.63 $\pm0.15$& 1.83 $\pm0.07$& 1.20\\
%    GConvNet &\xmark & \cmark   & 0.73 $\pm0.02$& 0.70 $\pm0.46$& 1.52 $\pm0.39$& 1.60 $\pm0.45$&1.14\\                Spherical UNet & %\xmark & \cmark  & 0.87 $\pm 1.44$& 2.90 $\pm0.52$& 2.19 $\pm0.38$& 2.57 $\pm0.02$ &2.13\\
%    MoNet & \xmark & \cmark  & 0.57 $\pm0.03$ & \textbf{0.57} $\pm0.02$&   1.33 $\pm0.21$&1.52 $\pm0.22$&1.00\\
%    \hline
%    SiT-tiny & \xmark & \cmark& 0.69 $\pm$ & 0.78 $\pm 5e^{-3}$ & 1.17 $\pm$0.06 & 1.36 $\pm$0.01&1.00\\
%    SiT-tiny &  \cmark& \cmark& 0.63 $\pm$0.01 & 0.67 $\pm$0.03 & 1.03 $\pm$0.09 & 1.31 $\pm$0.01&0.91\\
%    SiT-small &  \xmark& \cmark & 0.64 $\pm0.02$& 0.75 $\pm$0.01  & 1.14 $\pm$0.05& 1.22 $\pm$0.04&0.94\\
%    SiT-small &  \cmark& \cmark& 0.61 $\pm 1e^{-3}$& 0.71 $\pm$0.02& 1.02 $\pm$0.07& \textbf{1.21} $\pm$0.16&\textbf{0.89}\\
%    %\hline
%    %SiT-base  & \xmark& \xmark & 0.59 $\pm$& 0.68 $\pm$ & 1.11 $\pm$& 1.63 $\pm$\\
    %SiT-base  & \xmark& \cmark & 0. $\pm$& 0.71  $\pm$& 0. $\pm$& \textbf{1.21} $\pm$\\
    %SiT-base & \cmark& \xmark& 0.61 $\pm$& 0.70 $\pm$& 1.01 $\pm$& 1.60 $\pm$\\
    %SiT-base  & \cmark& \cmark & 0.58 $\pm$&  $\pm$& 0. $\pm$& 1.23 $\pm$\\
%    \hline
%    \hline
%  \end{tabular}
%  \caption{Optimised results of SiT - Best MAE is reported and standard deviations for the three best models.}  %we report Mean Average Error (MAE) in weeks (lower is better), for the best models. More details on training strategies are provided in \ref{appendix:hps-training-strategy}.}
%  \label{tab:results-vit}
%\end{table*}


%\begin{figure}[h]
%  \centering
%\makebox[\linewidth]{%to center the image
%	\includegraphics[width=1.0\columnwidth]{figures/maps.png}}
%\caption{Attention maps - HCP. [TO BE UPDATED FOLLOWING NEW RESULTS] Attention %maps overlaid on single subject parcellation maps for subjects with (a) high %and (b) low fluid intelligence scores. Multimodal parcellations and attention %maps are viewed on a very inflated for the left hemisphere only.}
%\label{figure:attention-map}
%\end{figure}


%Best performance over 5-folds cross validation was obtained using 50 ICA nodes and reported in Table \ref{Table:fluid_intelligence_results}. 
% a matrix reasoning test—a measure of fluid intelligence (gF)—was used as the phenotypic measure for prediction. In the HCP dataset, a 24-item version of the Penn Pro- gressive Matrices test was used; this test is an abbreviated form of Ra-ven’s standard progressive matrice
% In the HCP protocol, fluid intelligence (gF) was assessed using a form of Raven’s progressive matrices with 24 item, Bilker,  W.B. et  al.  Development  of  abbreviated  nine-item  forms  of  the  Raven’s Standard Progressive Matrices Test. Assessment 19, 354–369 (2012).


% \subsection{Surface Vision Transformers}

% % go into details
% In any case, patches are contiguous, non-overlapping but share common edges or vertex. The sequence of patches is first flattened into vectors where feature channels are concatenated per patch. The architecture the SiT is illustrated in Figure \ref{figure:sit}. The sequence of flattened vectors is projected into a sequence of dimension $D$ with a trainable linear layer. An extra vector of dimension $D$ is added to the sequence as an extra token, used for the regression. The SiT network is made of $L$ consecutive blocks of \textit{Multi-Head Self-Attention} (MHSA) and \textit{Feed Forward Network} (FFN) layers with residual connection between each layers. In the last output sequence, the regression token is used as input of the Multi-Layer Perceptron (MLP) head for prediction (regression or classification). 
% % explain the positional embedding. 


% projected into an embedding of dimension D via a trainable linear projection. % self-attention aims at capturing the interaction between the embeddings. There is therefore a tradeoff in how much information should each patch include. vs the lenght of the sequence. 

% explain in detail attention and self-attention mechanism. 

%\begin{figure}[!b]
%  \centering
%\makebox[\linewidth]{%to center the image
%	\includegraphics[width=1.0\columnwidth]{figures/surface_transformer.jpeg}}
%\caption{Surface Vision Transformers.}
%\label{figure:sit}
%\end{figure}


% This
% % %we extract contiguous triangular meshes defined on a ico-2 grid to form a sequence of cortical patches, 
% generates 320 patches, per hemisphere, and per channel. In all cases, before extracting patches, the right hemisphere is flipped to mirror the left orientation. Since there are four input channels (myelin, sulcal depth, curvature and cortical thickness) and the number vertices per patch is 153, the total dimension per patch is 612. %(see Appendix \ref{appendix:data} 

% variants of the vanilla ViT to mitigate the quadratic complexity with respect to the sequence size.
% segmentation: Organ than spread on large receptive field, multi-site segmentation (need context)
% various hybrid architectures have been developed to use feature extracted from both CNNs and transformers for medical image segmentation3 D volume segmentation, UNet like shape, with transformer encoder or attention layer to caputre local or globa context and CNN decoder,hybrid CNN-Transformer architecture to combine both local and global context.  Interpretable modelling.



% In \cite{M.Bronstein2021}, the transformer architecture is described as a particular instance of attentional Graph Neural Networks (GNN) over a complete graph, for which an ordering  between nodes is imposed by the use of positional embedding. 

% % Geometric deep learning in medical imaging
% In medical imaging, many geometric deep learning have been adapted to particularly in brain and cardiac imaging. 
% Obviously, geometric deep learning would benefit many medical related tasks to handle data that are inherently non-Euclidean: functional connectivity networks, medical imaging, surface analysis, omics data, molecular data.


% The SiT method in \cite{S.Dahan2022}, introduced a methodology for applying the vision transformers approaches to any surface data projected onto a genus-0 surface and demonstrated good performances in the context of cortical analysis. 

% transformers are becoming the generic architecture for preocessing sequential inputs. 


% capturing global-context in natural imaging datasets without the need for spatial priors in the architecture. This open the way for transformer to leverage the availability of very large datasets without being limited by the the convolution architectures/ 
% the cost of computing self
%Benefits of attention in computer vision tasks highlighted by \cite{ViT}.


%to become the de-facto architecture to use in natural imaging \cite{X.Chen2021,Z.Liu2022}, achieving competitive results and even improved on state-of-the-art results without relying on strong spatial priors: 

% Cerebral cortex is the highly convoluted outer surface of the brain, responsible for higher order cognitive and behavioural processes. 

%Accordingly, it would be advantageous if there could be a general framework that could perform consistently across tasks.

% Recently, \cite{A.Fawaz2021} benchmarked these methods for cortical phenotype regression and segmentation, and found solutions trade-off computational complexity, feature expressivity, and rotational equivariance, to generate very different solutions to the same biomedical problem, performing variably across different tasks. It would be advantageous if there could be a single unified geometric deep learning framework that could perform strongly across surface domains and across tasks.

%This mechanism of attention, already used in LSTM for language understanding \cite{J.Cheng2016}, learns how to create better representations of sequences by 

%function between token representations, and thus learning their relative importance within the sequence.

%that relies on a specific type of attention, the 

%these leveraged the scalability of the transformer architecture to be trained with 175 billions of parameters \cite{T.Brown2020} on 300 billion tokens from various web sources (Wikipedia, Common Crawl). 
% CNNs in general and medical imaging.

% the inductive biases of the convolution operation (scaling invariance, translation equivariance) has greatly contributed to this success. The 

%learn expressive filters capturing texture, edges or shapes. 


%to the the case for understanding neurological disorders, or relating distant regions for studying neurodevelopment. 
%and prevents leverage of rich/variable contextual information in very large datasets. 

%However, this locality property 

%CNNs with attention modules - discuss some examples. %\cite{M.Jaderberg2016, Wang2018, J.Hu2019}.

%voxel as a weighted average using the dot-product similarity of all feature maps voxels. 
%This concept of non-local mean is similar to the self-attention operation in NLP and demonstrated improvement in capturing long-range dependencies by learning information scattered across long-distant positions in successive frames.
%

%improving further medical image segmentation models \cite{AG.Roy2019}. 


%variants of spatial and channel-wise attention \cite{S.Jetley2018,J.Hu2019,Q.Wang2019,Y.Cao2019}, or guided attention \cite{O.Oktay2018,A.Sinha2019} but always restricted to low-resolution feature maps, in order to mitigate the cost. 
%have been adapted to medical image segmentation \cite{Z.Wang2018}, improving the modelling of global context in the encoder part compared to deep CNN encoders. + SE network for segmentation. SE gating mechanism to apply attention in the form of dynamic channel-wise feature recalibration. improve the modelling across channels. channel wise form of attention to highlight important feature dimension. Attention gate mechanisms to focus on specific part of feature maps to efficiently attend relevant information for specific tasks.  select salient image region the most information for to the specific task. \cite{J.Schlemper2018}
%Similarly, guided spatial and attention modules have been used in CNNs for medical imaging, to enrich the learning of contextual features especially for medical image segmentation \cite{O.Oktay2018,A.Sinha2019}.
% include global information (vs local neighbourhood)
% content-dependant interatctions, parameter independent- scaling of receptive field. https://arxiv.org/pdf/2103.12731.pdf

%between pertinent features at high spatial resolution.
% CNNs image-specific inductive biases, translation equivariance scaling invariance, modelling local features. Limited receptive field due to the locality property prevent for modelling long-range associations. 
% attention-driven vs attention-based methods
%Convolution-free attention-based computer vision models required a paradigm shift, where tasks such as image recognition are reformulated as a sequence-to-sequence type problem. 

%although CNNs have revolutionised performances for medical imaging tasks, their strong spatial priors restrain the modelling of global context necessary for some applications such as multi-organ segmentation or . Therefore, 

%with pure vision transformers or hybrid CNN/Transformers. %combining local and global contextual information. 
